Using the PALS Architecture to Verify a Distributed Topology Control Protocol for Wireless Multi-Hop Networks in the Presence of Node Failures

The PALS architecture reduces distributed, real-time asynchronous system design to the design of a synchronous system under reasonable requirements. Assuming logical synchrony leads to fewer system behaviors and provides a conceptually simpler paradigm for engineering purposes. One of the current limitations of the framework is that from a set of independent "synchronous machines", one must compose the entire synchronous system by hand, which is tedious and error-prone. We use Maude's meta-level to automatically generate a synchronous composition from user-provided component machines and a description of how the machines communicate with each other. We then use the new capabilities to verify the correctness of a distributed topology control protocol for wireless networks in the presence of nodes that may fail.

==> eptcsdata.tex <==
\providecommand{\firstpage}{101}
\providecommand{\publicationstatus}{P. C. \"Olveczky (Ed.): First International Workshop on\\
Rewriting Techniques for Real-Time Systems (RTRTS'10)\\
EPTCS 36, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.36.6}{10.4204/EPTCS.36.6}}
\pdfoutput=1

